On the diversity and frequency of code related to mathematical formulas in real-world Java projects

In this paper, the term formula code refers to fragments of source code that implement a mathematical formula. We present empirical studies that analyze the diversity and frequency of formula code in open-source-software projects. In an exploratory study, we investigated what kinds of formulas are implemented in real-world Java projects and derived syntactical patterns and constraints. We refined these patterns for sum and product formulas to automatically detect formula code in software archives and to reconstruct the implemented formula in mathematical notation. In a quantitative study of a large sample of engineered Java projects on GitHub we analyzed the frequency of formula code and estimated that one of 700 lines of code in this sample implements a sum or product formula. For a sample of scientific-computing projects, we found that one of 100 lines of code implements a sum or product formula. To assess the need for tool support, we investigated the helpfulness of comments for program understanding in a sample of formula-code fragments and performed an online survey. Our findings provide first insights into the characteristics of formula code, that can motivate further studies on the role of formula code in software projects and the design of formula-related tools.

==> sections/formula-code-detection-tool.tex <==
To automate the search for formula code, in particular SP-formula code, we developed a detection tool which utilizes the patterns and corresponding constraints introduced in Section ~\ref{patterns:sec}. First, the user
has to select the GitHub repositories to be analyzed. The default branches of these repositories are then automatically checked out and saved locally by the tool. Next, 
all Java files in these projects are read one after another (comments in the
source code are removed) and searched for all patterns in parallel to exploit multiple CPU cores. 
\attic{
by using one thread per file testing all patterns.
}
Each pattern is implemented as a regular expression.
\attic{
and further compiled into an automaton
by using the {\tt java.util.regex} library.
}
The \attic{resulting pattern matcher} tool also captures and pre-processes pattern-specific elements like variable roles, such that the constraints associated with each pattern can be tested. Matched code fragments that satisfy the constraints are attached to the output which is stored in form of a CSV file. This file lists for each entry, the line numbers start and end of the match, the source code of the code fragments, the inferred formula in mathematical notation (both in a textual representation as well as in MathML, basically an instance of our formula templates) as well as other detailed information about the source like project name, file name and GitHub path.

\attic{ 
\todo{SD: OO-Implementierungsdetails sind uninteressant, das ist Handwerkszeug}
Each of the elaborated schemes is created as an own class and is worded as regular expression according to the java.util.regex library. Besides, each scheme contains a matcher as inner class which acts as indicator and controls the pattern-specific output (among others the automated readout of the equivalent mathematical notation). To reuse matched elements of the patterns they get captured with the aid of capturing groups, which is a feature of the corresponding library. Storing them into variables allows performing the various tests afterwards. Since the tests are generally worded, so that they are valid for each for-loop pattern, capturing and storing these captured elements can be done at a higher level than that one of the indicators by use of a superior class named ForloopCaptor. This one interacts with the ForloopTester so that it can be determined whether the considered pattern satisfies the requirements and should be added to the output.
Three abstract super classes (in each case one for the patterns, the matchers and the testers) serve as structural elements in the class hierarchy by presetting attributes and methods. By implementing concrete methods on the other hand these classes and their subclasses are getting integrated into the program run. Through these generalized super classes one can add further schemes to the tool analogously to the for-loop patterns.
}

Listing~\ref{regularexp:lst} shows the regular expression 
for Pattern~\ref{sumforpattern:pat} (all patterns available in the supplementary material ~\cite{moseler_oliver_2018_1252324}). Note that the regular expression 
is built using String constants like {\tt VAR} and {\tt EXP} which 
contain themselves regular expressions:
\begin{center}
\setcounter{lstlisting}{2}
\begin{lstlisting}[language=Java,mathescape=true,escapeinside={(*}{*)},basicstyle=\small\ttfamily,caption=Regular expression for non-nested \texttt{for}-loop implementing a sum/procuct  (Pattern~\ref{sumforpattern:pat}),label=regularexp:lst]
Pattern.compile(
 (*\color{blue}{// head of loop}*)
 "(?<lineOuterFor>for"+b+"\\((?:"+b+DT+b2+")?"+
 "(?<ind0>"+VAR+")"+b+"="+b+"(?<exp00>"+EXP+")"+
 b+";"+b+"\\k<ind0>"+b+"(?<relOp0>"+REL_OP+")"+b+
 "(?<exp10>"+EXP+")"+b+";"+ITER0_INCREASE+"\\))\\s*+"
 (*\color{blue}{// body in brackets}*)				
 + "(?:\\{\\s*?" + 
   "(?<blockFiOu>"+BLOCKR+"\\s++)" + 
   "(?<lineAssiA>"+ACCUA_ASSIGNMENT+";)\\s*+" +
   "(?<blockSeOu>"+BLOCKP+")\\s*+" +
   "\\}"
 (*\color{blue}{// no brackets}*)							
 + "|" +
   "(?<lineAssiB>"+ACCUB_ASSIGNMENT+";))");
\end{lstlisting}
\end{center}

\attic{Given the diversity of the formulas that we found, we decided to focus on sum and product formulas for our
quantitative analysis, because they are non-trivial and we expected them to occur quite frequently.} 
\attic{Thus,} We implemented the 10 patterns
listed in Table~\ref{patterntypes:tab} to detect SP-formula code. 
On average, the regular expressions for non-nested loops consist 
of 8 lines of code without comments, those for nested loops of 28 lines.

%non-nested {\tt for}-loop for sum/product,
%non-nested {\tt foreach}-loop for sum/product,
%non-nested {\tt for}-loop for arrays,
%non-nested {\tt foreach}-loop for arrays/collections, 
%nested {\tt for}-loops for sum/product of sums/products,
%nested {\tt foreach}-loops for sum/product of sums/products,
%nested {\tt for}-loops for array of products/sums,
%nested {\tt foreach}-loops for array/collection of products/sums,
%nested {\tt for}-loops for array of arrays,
%nested {\tt foreach}-loops for array/collection of arrays/collections.
  

%NON-Commented lines of code der reg. Ausdrücke
%FIA 8 NCLOC
%FEA 9 NCLOC
%FIS 8 NCLOC
%FES 8 NCLOC
%FISS 28 NCLOC
%FESS 28 NCLOC
%FIAS 28 NCLOC
%FEAS 27 NCLOC
%FIAA 28 NCLOC
%FEAA 28 NCLOC


%For the present it is based on the derived for-loop patterns, but henceforth can be extended with further formula code schemes.
 %%{\sf FIS}
\attic{
\begin{description}[align=left, font=\normalfont\normalcolor\sffamily] %\label{patterntypes:desc}
\item [FIS:] non-nested {\tt for}-loop for sum/product
\item [FES:] non-nested {\tt foreach}-loop for sum/product
\item [FIA:] non-nested {\tt for}-loop for arrays
\item [FEC:] non-nested {\tt foreach}-loop for arrays/collections
\item [NFISS:] nested {\tt for}-loops for sum/product of sums/products
\item [NFESS:] nested {\tt foreach}-loops for sum/product of sums/products
\item [NFIAS:] nested {\tt for}-loops for array of products/sums
\item [NFECS:] nested {\tt foreach}-loops for array/collection of products/sums
\item [NFIAA:] nested {\tt for}-loops for array of arrays
\item [NFECC:] nested {\tt foreach}-loops for array/collection of arrays/collections
\end{description}
}

\begin{table}
\caption{Patterns implemented by the tool~\label{patterntypes:tab}}
\begin{tabular}{>{\sf}l>{\small}l}
     & {\normalsize Patterns for non-nested loops}\\
 \hline
 FIS & {\tt for}-loop for sum/product\\
 FES & {\tt foreach}-loop for sum/product\\
 FIA & {\tt for}-loop for arrays\\
 FEC & {\tt foreach}-loop for arrays/collections\\
 \\
    & {\normalsize Patterns for nested loops}\\
 \hline
 NFISS & {\tt for}-loops for sum/product of sums/products\\
 NFESS & {\tt foreach}-loops for sum/product of sums/products\\
 NFIAS & {\tt for}-loops for array of products/sums\\
 NFECS & {\tt foreach}-loops for array/collection of products/sums\\
 NFIAA & {\tt for}-loops for array of arrays\\
 NFECC & {\tt foreach}-loops for array/collection of arrays/collections\\
\hline
\end{tabular}
\end{table}

\subsection{Evaluation}\label{evaluation:sec}

%We performed a case study to assess the quality of our formula mining tool in terms of recall and precision.

To evaluate our approach to detect SP-formula code in software repositories 
we applied our tool with the patterns listed in Table~\ref{patterntypes:tab} 
to random samples of Java files on GitHub.
As validation metrics we use recall and precision:
\begin{itemize}
\item How many of the SP-formula code fragments in a sample 
      are automatically detected?
\item To what extent are the detected SP-formula code fragments correct?
\end{itemize}
% The estimation of the quality in form of precision and recall was of interest.

More precisely, let $F$ be the set of all formula code fragments in the sample,
and $D$ be the detected formula code fragments. Then the recall is the number of correctly found formula code fragments divided by all all correct formula code fragments, i.e., ${\sf recall} = \frac{|D\cap F|}{|F|}$, and the precision
is the number of correctly found formula code fragments divided by all found 
formula code fragments, i.e., ${\sf precision} = \frac{|D\cap F|}{|D|}$.

\attic{
\todo{SD: Das stimmt ja so nicht, da wir in der Studie watcher $>$ 10 nehmen:
Since there are no sufficient studies about the quality, properties and characteristics of the data available on GitHub, there do not exist any guidelines to chose adequate samples%~\cite{kalliamvakou2014promises}\todo{OM:  Ist die Referenz so ok?}.
}
}

With the aid of Google Big Query and the GHTorrent data set, we computed a list 
of 21,052,682 Java files on GitHub. The list does not include any forked repositories
and duplicates, i.e. files with the same hash value. 
%This sample keeps the universe's characteristics and maintains the representativeness for all GH repositories (not only for the relevant ones). There are no limitations in our approach except the avoiding of forks and file duplicates. 
%In this way we created a representative data set that can serve as basis for many studies by determining an adequate sample size and pulling without replacement. 

To draw random samples from the above data set we used R. \attic{ and its uniform distributed function `runif'.} To measure the recall of our approach we used a sample of 1,000 Java files, to measure its precision we used a sample 
of 10,000 files. 
%%
Since GHTorrent is an off-line mirror of GitHub, it can contain files 
which have already been moved, removed, renamed on GitHub. 
%there aren't all files frequently synchronized and updated at , 
Thus, we could not download the source code of all drawn files from GitHub 
and the real sample sizes came to 878 and 8,960. 
%For both measures the tool was executed with the respective sample. 


\paragraph{Oracle} For computing the recall, we created an oracle data set
by manually inspecting the complete sample of 878 files and 
annotating the formula code fragments that we found. We annotated the code fragments in a group discussion in order to reduce subjective biases.
%in the, for our situation, highest extent achievable. 
To annotate the fragments, we enclosed them in XML-tags which can be nested. The choice of 
the tags {\small\verb+<SimpleNestedLoop>+}, {\small\verb+<DoubleNestedLoop>+}, %{\small\verb+<SimpleFormula>+}, {\small\verb+<Assignment>+},
{\small\verb+<SimpleArithmetic>+},
{\small\verb+<Matrix>+}, and {\small\verb+<Vector>+} is based on the results of our keyword-based search. Finally,
we manually found and annotated 145 formula code fragments in 53 
of the 878 files (6.04\%). These formula code fragments 
made up 1,064 lines of 142,419 total lines of code (0.75\%).
These annotated formula code fragments contained SP-formula code
% loops {\small\verb+<SimpleNestedLoop>+} or {\small\verb+<DoubleNestedLoop>+} 
in 110 cases (75.86\%). 
Almost all remaining cases were annotated with %{\small\verb+<SimpleFormula>+}
{\small\verb+<SimpleArithmetic>+} 
which we used to describe simple, but non-trivial arithmetic expressions. The mathematical representation of those expressions may have some added value compared to 
the representation in program code, 
e.g. $\sqrt{5}$ instead of {\small\verb+Math.sqrt(5)+}.
%\todo{SD: Stimmt das Beispiel mit der Wurzel ???}
%expressions that have some added value are  whose notation as mathematical pendant creates an added value. 
Matrices and vectors were only used in 4 lines outside of loops.
%There were 50 loops with 'Assignments', such as accumulators or arrays like in our derived patterns. 


\paragraph{Recall}
%Now the recall can be measured as share of identified for-loop patterns in for-loop patterns generally or in formula code generally.
Our tool found 34 correct SP-formula code fragments in the oracle data set.  
Thus, %the recall relating to formula code in general amounts to 23.45\%, whereas 
the recall is 30.91\%. % if we only consider the loop formula code in the oracle data set, see Figure~\ref{toolrecall:fig}.  
In cases where both the inner and the outer loop where
detected, it makes sense to only consider the outer one.
Fortunately, in our evaluation this case never happened.

\attic{
\begin{figure}[ht]
	\centering
	\caption{Recall of the Formula Code Mining Tool\label{toolrecall:fig}}
	\includegraphics[scale=1]{./images/Recall}
	%	\label{fig1}
\end{figure}
}

%Examining the output yields the recall by comparing it to the dispersions of the sample's universe.

\paragraph{Precision}
To measure the precision we applied our tool to the 
8,960 Java files of the second, non-annotated sample. For each detected
formula code fragment, we manually checked whether the matched
code fragment implemented a SP-formula. We also recorded whether the inferred formula covered the complete formula code 
or only a part of it.
%Furthermore, in the former case one can differentiate if the indication of the mathematical formula is correct and describes the complete formula code, if it is correct, but not perfect or if it is wrong. 

Our tool found 181 matches. All of these matches contained SP-formula code. 153 code fragments got completely specified by the inferred formula. 
For 23 matches the tool inferred a correct formula that, however, did not describe the whole code excerpt. 
Only in 5 cases we found that the inferred mathematical formula was
inadequate or wrong (2.76\%). %% SD: wrong heisst nicht false positive !!! 
Thus,\attic{ as shown in Figure~\ref{toolprecision:fig},}
if we only take into account whether
the match contained formula code, the precision was 100\%. 
If we require that the inferred formula is correct, the precision
was 97.24\%, and if we require that the inferred formula is correct 
and completely describes the effect of the code matched, the precision
was 84.53\%.

\attic{
\begin{figure}[ht]
	\centering
	\caption{Precision of the SP-Formula-Code Detection\label{toolprecision:fig}}
	\includegraphics[scale=1]{./images/Precision}
	%	\label{fig1}
\end{figure}
}

\paragraph{Formula code density} To quantify how often formula
code occurs in real world software (RQ2), we define two different 
measures for the formula code density---one
based on lines of codes $\rho_{LOC}$
and one based on number of unique files $\rho_{files}$:
\begin{eqnarray} \label{fcdensityfiles:equ}
\rho_{files} = \frac{\mbox{\#files containing formula code}}{\mbox{\#all scanned files}}\\
\rho_{LOC} = \frac{\mbox{\#lines with formula code in all scanned files}}{\mbox{\#lines of all scanned files}}\label{fcdensityloc:equ}
\end{eqnarray}

\attic{
Figure~\ref{oracleFCdensity:fig} shows the formula code 
density in our oracle data set, i.e. based on all manually 
identified and annotated formula code fragments.
}
% Furthermore, it can serve as basis for extrapolations in projects.
% \rho_{files} = 6.04 \% , \rho_{lines}=0.75\%

%\todo{SD: Die Abbildung zeigt nicht die Dichte, sondern die absoluten Werte.}

%\todo{SD: Figure 3 koennten wir auch einfach durch Text ersetzen: }
The formula code densities in our oracle data set, i.e. based on all manually 
identified and annotated formula code fragments, were
$\rho_{files}=\frac{53}{878}= 6.04\%$ and
$\rho_{LOC}=\frac{1,064}{142,419}= 0.76\%$. In other words,
in our oracle data set on average
one of 130 lines of code was part of an implementation
of a formula.

\attic{
\begin{figure}[ht]
	\centering
	\caption{Formula Code Density in Oracle Data Set\label{oracleFCdensity:fig}}
	%\includegraphics[scale=1]{./images/FormulaCodeDensity}
    \includegraphics[scale=.9]{./images/oracleFormulaDensity}
	%	\label{fig1}
\end{figure}
}

 

%\subsubsection{Creation of an Oracle}

